Emergent spin-charge-orbital order in superconductor La$_3$Ni$_2$O$_7$

The bilayer nickelate La$_3$Ni$_2$O$_7$ (LNO) exhibits a remarkably high-temperature superconductivity of approximately 80 K under pressure, sparking considerable attentions. However, the nature of the spin, charge, and orbital order in LNO remains unknown, hindering the exploration of the mechanism of superconductivity. Here, supported by symmetry analysis and density functional theory calculations, we unravel a double strip ground state of LNO with alternating magnetic moments arrangements. Interestingly, a charge density wave emerges under this determined magnetic order. Such CDW phase exhibits a Pmnm space group with breathing deformation of the NiO$_6$ octahedra, where the stretching and shrinking of the octahedra correspond to the formation of \emph{d}$_{z^2}^1$\emph{d}$_{x^2-y^2}^1$ and \emph{d}$_{z^2}^1$ orbital order. Moreover, we build a first-principles-based Hamiltonian for LNO, which provides deeper insight into its peculiar magnetic order. Our work thus reveals a systematic spin-charge-orbital picture for LNO, which can be extended to other nickelate-based superconductors, paving the way for determining the mechanism of superconductivity.

==> bib.tex <==
% Generated by IEEEtran.bst, version: 1.14 (2015/08/26)
\begin{thebibliography}{10}
\providecommand{\url}[1]{#1}
\csname url@samestyle\endcsname
\providecommand{\newblock}{\relax}
\providecommand{\bibinfo}[2]{#2}
\providecommand{\BIBentrySTDinterwordspacing}{\spaceskip=0pt\relax}
\providecommand{\BIBentryALTinterwordstretchfactor}{4}
\providecommand{\BIBentryALTinterwordspacing}{\spaceskip=\fontdimen2\font plus
\BIBentryALTinterwordstretchfactor\fontdimen3\font minus \fontdimen4\font\relax}
\providecommand{\BIBforeignlanguage}[2]{{%
\expandafter\ifx\csname l@#1\endcsname\relax
\typeout{** WARNING: IEEEtran.bst: No hyphenation pattern has been}%
\typeout{** loaded for the language `#1'. Using the pattern for}%
\typeout{** the default language instead.}%
\else
\language=\csname l@#1\endcsname
\fi
#2}}
\providecommand{\BIBdecl}{\relax}
\BIBdecl

\bibitem{chen2024evidence}
K.~Chen, X.~Liu, J.~Jiao, M.~Zou, C.~Jiang, X.~Li, Y.~Luo, Q.~Wu, N.~Zhang, Y.~Guo \emph{et~al.}, ``Evidence of spin density waves in la 3 ni 2 o 7-$\delta$,'' \emph{Physical Review Letters}, vol. 132, no.~25, p. 256503, 2024.

\bibitem{zhang2024high}
Y.~Zhang, D.~Su, Y.~Huang, Z.~Shan, H.~Sun, M.~Huo, K.~Ye, J.~Zhang, Z.~Yang, Y.~Xu \emph{et~al.}, ``High-temperature superconductivity with zero resistance and strange-metal behaviour in la3ni2o7- $\delta$,'' \emph{Nature Physics}, pp. 1--5, 2024.

\bibitem{li2024electronic}
Y.~Li, X.~Du, Y.~Cao, C.~Pei, M.~Zhang, W.~Zhao, K.~Zhai, R.~Xu, Z.~Liu, Z.~Li \emph{et~al.}, ``Electronic correlation and pseudogap-like behavior of high-temperature superconductor la3ni2o7,'' \emph{Chinese Physics Letters}, 2024.

\bibitem{sun2023signatures}
H.~Sun, M.~Huo, X.~Hu, J.~Li, Z.~Liu, Y.~Han, L.~Tang, Z.~Mao, P.~Yang, B.~Wang \emph{et~al.}, ``Signatures of superconductivity near 80 k in a nickelate under high pressure,'' \emph{Nature}, vol. 621, no. 7979, pp. 493--498, 2023.

\bibitem{dan2024spin}
Z.~Dan, Y.~Zhou, M.~Huo, Y.~Wang, L.~Nie, M.~Wang, T.~Wu, and X.~Chen, ``Spin-density-wave transition in double-layer nickelate la3ni2o7,'' \emph{arXiv preprint arXiv:2402.03952}, 2024.

\bibitem{zhang2024structural}
Y.~Zhang, L.-F. Lin, A.~Moreo, T.~A. Maier, and E.~Dagotto, ``Structural phase transition, s$\pm$-wave pairing, and magnetic stripe order in bilayered superconductor la3ni2o7 under pressure,'' \emph{Nature Communications}, vol.~15, no.~1, p. 2470, 2024.

\bibitem{yang2024orbital}
J.~Yang, H.~Sun, X.~Hu, Y.~Xie, T.~Miao, H.~Luo, H.~Chen, B.~Liang, W.~Zhu, G.~Qu \emph{et~al.}, ``Orbital-dependent electron correlation in double-layer nickelate la3ni2o7,'' \emph{Nature Communications}, vol.~15, no.~1, p. 4373, 2024.

\bibitem{yu2024density}
X.~H. Yu, Y.~Meng, Y.~Yang, H.~Sun, S.~Zhang, J.~Luo, L.~Chen, X.~Ma, M.~Wang, F.~Hong \emph{et~al.}, ``Density-wave-like gap evolution in la3ni2o7 under high pressure revealed by ultrafast optical spectroscopy,'' 2024.

\bibitem{chen2024electronic}
X.~Chen, J.~Choi, Z.~Jiang, J.~Mei, K.~Jiang, J.~Li, S.~Agrestini, M.~Garcia-Fernandez, H.~Sun \emph{et~al.}, ``Electronic and magnetic excitations in la3ni2o7,'' 2024.

\bibitem{khasanov2024pressure}
R.~Khasanov, T.~J. Hicken, D.~J. Gawryluk, L.~P. Sorel, S.~B{\"o}tzel, F.~Lechermann, I.~M. Eremin, H.~Luetkens, and Z.~Guguchia, ``Pressure-induced split of the density wave transitions in la $ \_3 $ ni $ \_2 $ o $ \_ $\{$7-$\backslash$delta$\}$ $,'' \emph{arXiv preprint arXiv:2402.10485}, 2024.

\bibitem{zhang2020intertwined}
J.~Zhang, D.~Phelan, A.~Botana, Y.-S. Chen, H.~Zheng, M.~Krogstad, S.~G. Wang, Y.~Qiu, J.~Rodriguez-Rivera, R.~Osborn \emph{et~al.}, ``Intertwined density waves in a metallic nickelate,'' \emph{Nature communications}, vol.~11, no.~1, p. 6003, 2020.

\bibitem{ling2000neutron}
C.~D. Ling, D.~N. Argyriou, G.~Wu, and J.~Neumeier, ``Neutron diffraction study of la3ni2o7: Structural relationships among n= 1, 2, and 3 phases lan+ 1nino3n+ 1,'' \emph{Journal of Solid State Chemistry}, vol. 152, no.~2, pp. 517--525, 2000.

\bibitem{liu2023evidence}
Z.~Liu, H.~Sun, M.~Huo, X.~Ma, Y.~Ji, E.~Yi, L.~Li, H.~Liu, J.~Yu, Z.~Zhang \emph{et~al.}, ``Evidence for charge and spin density waves in single crystals of la3ni2o7 and la3ni2o6,'' \emph{Science China Physics, Mechanics \& Astronomy}, vol.~66, no.~1, p. 217411, 2023.

\bibitem{wang2024structure}
L.~Wang, Y.~Li, S.-Y. Xie, F.~Liu, H.~Sun, C.~Huang, Y.~Gao, T.~Nakagawa, B.~Fu, B.~Dong \emph{et~al.}, ``Structure responsible for the superconducting state in la3ni2o7 at high-pressure and low-temperature conditions,'' \emph{Journal of the American Chemical Society}, vol. 146, no.~11, pp. 7506--7514, 2024.

\bibitem{luo2023bilayer}
Z.~Luo, X.~Hu, M.~Wang, W.~W{\'u}, and D.-X. Yao, ``Bilayer two-orbital model of l a 3 n i 2 o 7 under pressure,'' \emph{Physical review letters}, vol. 131, no.~12, p. 126001, 2023.

\bibitem{christiansson2023correlated}
V.~Christiansson, F.~Petocchi, and P.~Werner, ``Correlated electronic structure of la 3 ni 2 o 7 under pressure,'' \emph{Physical Review Letters}, vol. 131, no.~20, p. 206501, 2023.

\bibitem{zhu2023superconductivity}
Y.~Zhu, E.~Zhang, B.~Pan, X.~Chen, D.~Peng, L.~Chen, H.~Ren, F.~Liu, N.~Li, Z.~Xing \emph{et~al.}, ``Superconductivity in trilayer nickelate la $ \_4 $ ni $ \_3 $ o $ \_ $\{$10$\}$ $ single crystals,'' \emph{Nature}, vol. 631, p. 531–536, 2024.

\bibitem{hou2023emergence}
J.~Hou, P.-T. Yang, Z.-Y. Liu, J.-Y. Li, P.-F. Shan, L.~Ma, G.~Wang, N.-N. Wang, H.-Z. Guo, J.-P. Sun \emph{et~al.}, ``Emergence of high-temperature superconducting phase in pressurized la3ni2o7 crystals,'' \emph{Chinese Physics Letters}, vol.~40, no.~11, p. 117302, 2023.

\bibitem{zhang2023electronic}
Y.~Zhang, L.-F. Lin, A.~Moreo, and E.~Dagotto, ``Electronic structure, dimer physics, orbital-selective behavior, and magnetic tendencies in the bilayer nickelate superconductor la 3 ni 2 o 7 under pressure,'' \emph{Physical Review B}, vol. 108, no.~18, p. L180510, 2023.

\bibitem{sakakibara2024possible}
H.~Sakakibara, N.~Kitamine, M.~Ochi, and K.~Kuroki, ``Possible high t c superconductivity in la 3 ni 2 o 7 under high pressure through manifestation of a nearly half-filled bilayer hubbard model,'' \emph{Physical Review Letters}, vol. 132, no.~10, p. 106002, 2024.

\bibitem{lu2024interlayer}
C.~Lu, Z.~Pan, F.~Yang, and C.~Wu, ``Interlayer-coupling-driven high-temperature superconductivity in la 3 ni 2 o 7 under pressure,'' \emph{Physical Review Letters}, vol. 132, no.~14, p. 146002, 2024.

\bibitem{qu2024bilayer}
X.-Z. Qu, D.-W. Qu, J.~Chen, C.~Wu, F.~Yang, W.~Li, and G.~Su, ``Bilayer t-j-j⊥ model and magnetically mediated pairing in the pressurized nickelate la 3 ni 2 o 7,'' \emph{Physical Review Letters}, vol. 132, no.~3, p. 036502, 2024.

\bibitem{liu2023s}
Y.-B. Liu, J.-W. Mei, F.~Ye, W.-Q. Chen, and F.~Yang, ``s$\pm$-wave pairing and the destructive role of apical-oxygen deficiencies in la 3 ni 2 o 7 under pressure,'' \emph{Physical Review Letters}, vol. 131, no.~23, p. 236002, 2023.

\bibitem{SM}
See Supplemental Material at http://link for more information, which includes {Refs}. \cite{perdew1996generalized,kresse1996efficiency,kresse1996efficient2,blochl1994projector,grimme2010consistent,togo2015first,wang2021vaspkit}.

\bibitem{wang2021vaspkit}
V.~Wang, N.~Xu, J.-C. Liu, G.~Tang, and W.-T. Geng, ``{VASPKIT}: A user-friendly interface facilitating high-throughput computing and analysis using {VASP} code,'' \emph{Comput. Phys. Commun.}, vol. 267, p. 108033, 2021.

\bibitem{perdew1996generalized}
J.~P. Perdew, K.~Burke, and M.~Ernzerhof, ``Generalized gradient approximation made simple,'' \emph{Phys. Rev. Lett.}, vol.~77, no.~18, p. 3865, 1996.

\bibitem{kresse1996efficiency}
G.~Kresse and J.~Furthm{\"u}ller, ``Efficiency of \emph{ab-initio} total energy calculations for metals and semiconductors using a plane-wave basis set,'' \emph{Comput. Mater. Sci.}, vol.~6, no.~1, pp. 15--50, 1996.

\bibitem{kresse1996efficient2}
G.~Kresse and J.~Furthm\"uller, ``Efficient iterative schemes for \emph{ab initio} total-energy calculations using a plane-wave basis set,'' \emph{Phys. Rev. B}, vol.~54, no.~16, p. 11169, 1996.

\bibitem{blochl1994projector}
P.~E. Bl{\"o}chl, ``Projector augmented-wave method,'' \emph{Phys. Rev. B}, vol.~50, no.~24, p. 17953, 1994.

\bibitem{grimme2010consistent}
S.~Grimme, J.~Antony, S.~Ehrlich, and H.~Krieg, ``A consistent and accurate ab initio parametrization of density functional dispersion correction {(DFT-D)} for the 94 elements {H-Pu},'' \emph{J. Chem. Phys.}, vol. 132, no.~15, p. 154104, 2010.

\bibitem{togo2015first}
A.~Togo and I.~Tanaka, ``First principles phonon calculations in materials science,'' \emph{Scr. Mater.}, vol. 108, pp. 1--5, 2015.

\end{thebibliography}

